Channel Selection for Network-assisted D2D Communication via No-Regret Bandit Learning with Calibrated Forecasting

We consider the distributed channel selection problem in the context of device-to-device (D2D) communication as an underlay to a cellular network. Underlaid D2D users communicate directly by utilizing the cellular spectrum but their decisions are not governed by any centralized controller. Selfish D2D users that compete for access to the resources construct a distributed system, where the transmission performance depends on channel availability and quality. This information, however, is difficult to acquire. Moreover, the adverse effects of D2D users on cellular transmissions should be minimized. In order to overcome these limitations, we propose a network-assisted distributed channel selection approach in which D2D users are only allowed to use vacant cellular channels. This scenario is modeled as a multi-player multi-armed bandit game with side information, for which a distributed algorithmic solution is proposed. The solution is a combination of no-regret learning and calibrated forecasting, and can be applied to a broad class of multi-player stochastic learning problems, in addition to the formulated channel selection problem. Analytically, it is established that this approach not only yields vanishing regret (in comparison to the global optimal solution), but also guarantees that the empirical joint frequencies of the game converge to the set of correlated equilibria.

==> LaTeX1.tex <==
Consider a selection strategy $\kappa$ so that any player $k$ plays by actions $m_{k,t}=g(\delta_{d_{t}})$, where $\delta_{d_{t}}$ is the dirac probability distribution on the true joint action profile of its opponets at time $t$, and $g$ is some rule (such as best response) that guarantees
%
\begin{equation}
\label{eq:lmConOne}
\lim_{T \to \infty} S_{\kappa,T} = \lim_{T \to \infty} \frac{\sum_{t=1}^{T}f_{m_{k,t},k}(k^{-}_{t})}{\sum_{t=1}^{T}f^{*}_{k}(k^{-}_{t})}=1.
\end{equation}
\end{equation}
%
Then if player $k$ plays using another selection strategy $\kappa'$ so that $m_{k,t}=g(P_{t})$, where $P_{t}$ is a probability distribution over all possible joint action profile of its opponnets produced by a calibrated forecaster, we have
%
\begin{equation}
\label{eq:lmConOne}
\lim_{T \to \infty} S_{\kappa',T} = \lim_{T \to \infty} \frac{\sum_{t=1}^{T}f_{m_{k,t},k}(k^{-}_{t})}{\sum_{t=1}^{T}f^{*}_{k}(k^{-}_{t})}=1.
\end{equation}
\end{equation}
%
In other words, if a strategy is strongly consistent given true joint action profiles, then its consistency is preserved even by using the predicted joint action profiles, provided that the forecaster is calibrated. 

%TTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTTheorem 4



Consider a K_player MAB game where each palyer is provided with $M$ actions. Let $\mathfrak{C}$ denote the set of correlated equilbria, $\textbf{m}=(m_{1},..,m_{K})\in \bigotimes_{k=1}^{K}\left \{ 1,..,M \right \}$, and define the empirical joint frequencies of paly as (\ref{eq:empiricalFreq}). If all players play according to sellection strategy $\chi$, then the distance $\inf_{\pi \in \mathfrak{C}}\sum_{\textbf{m}}\left | \hat{\pi}_{T}(\textbf{m}) -\pi(\textbf{m})\right |$ between the empirical joint distribution of plays and the set of correlated equilibria converges to $0$ almost surely as $T \to \infty$.  

%----------------------------Proof-------------------------------------------------------




Consider a K-player MAB game, as described in Section \ref{subsec:MP_MAB}. By Theorem \ref{th:CorrConvergence}, if each player plays by best responding to a calibrated forecast of the joint action profile of opponents, then we have $\lim_{T \to \infty} \inf_{\pi \in \mathfrak{C}}\sum_{\textbf{m}}\left | \hat{\pi}_{T}(\textbf{m}) -\pi(\textbf{m})\right | =0$. We refer to this selection strategy as $\chi'$. In order to prove the Theorem, we need to show that our selection strategy $\chi$, in which the true expected rewards of joint action profiles are not known and they should be learned by exploration, exhibits the same convergence characteristics as $\chi'$. 

First, we re-arrange the K-player MAB game to a two-agent game where the first agnet is any palyer $k$ and the second agent is the set of all its opponets, i.e. the set of $K-1$ players. For this game, any joint action profiles of the two agents can be written as $(m,\textbf{m'})$, where $m \in {1,...,M}$ and $\textbf{m'} \in \bigotimes_{k=1}^{K-1}\left \{1,...,M \right \}$. Let $\tau_{T}(m,\textbf{m'})$ denote the farction of trials until time $T$ in which some joint action $(m,\textbf{m'})$ is played. According to selection strategy $\chi$, $\Gamma_{T}(m,\textbf{m'})$ can be written as 
%
\begin{equation}
\label{eq:farction}
\Gamma_{T}(m,\textbf{m'})=\Gamma_{T,r}(m,\textbf{m'})+\Gamma_{T,i}(m,\textbf{m'}),
\end{equation}
%
where $\Gamma_{T,r}(m,\textbf{m'})$ and $\Gamma_{T,i}(m,\textbf{m'})$ denote the fractions of trials in which $(m,\textbf{m'})$ is palyed by exploration (i.e. by chance), and by exploitation (i.e. according to the best response rule given by (\ref{eq:BestResponse})), respectively. According to Algorithm \ref{alg:Selection}, the total number of exploration trials is given by $\sum_{r=1}^{R}\left \lceil T'_{r}Z_{r} \right \rceil$. Moreover, by Assumption \ref{as:bandit_game}, we know 
%
\begin{equation}
\lim_{R \to \infty} \frac{\sum_{r=1}^{R}\left \lceil T'_{r}Z_{r} \right \rceil}{\sum_{r=1}^{R}T'_{r}}=0.
\end{equation}
%
This implies that
\begin{equation}
\label{eq:farctionTwo}
\lim_{T \to \infty}~~\Gamma_{T,r}(m,\textbf{m'})=0,
\end{equation}
%
Therefore, asympthotically, $\Gamma_{T,r}(m,\textbf{m'})$ can be neglected when calculating the empirical frequencies of plays, and hence
%
\begin{equation}
\label{eq:farctionThree}
\lim_{T \to \infty}~~\Gamma_{T}(m,\textbf{m'})=\Gamma_{T,i}(m,\textbf{m'}).
\end{equation}
%

In order to complete the proof, it is sufficient to show that after some finite time, the actions taken by the player based on $\hat{f}_{m,k,t}$ are equal to those based on $f_{m,t}$. By Assumption \ref{as:expected_reward}, we know that, with probability 1, there exists an $\nu>0$ so that for every $m \in \left \{1,...,M \right \}$, after a time point $\theta<\infty$, 
%
\begin{equation}
\label{eq:Conv-Lemma}
\|\hat{f}_{m,k}(k^{-})-f_{m,k}(k^{-})\|<\nu,
\end{equation}
%
holds for all $t>\theta$. At the same time, according to our system model and by Assumption \ref{as:expected_reward}, the reward functions are bounded, and the action space and memory are finite. This implies that if (\ref{eq:Conv-Lemma}) holds, then the actions of the player evolve as if the player were aware of the true expected reward of each joint action profile, which completes the proof. 





==> lm-assumption.tex <==
\subsection{Proof of Lemma \ref{lm:Assumption}}\label{subsec:lm_Assumption}
%---------------------------------------------------------------------------------
